Concept-Based Embeddings for Natural Language Processing

In this work, we focus on effectively leveraging and integrating information from concept-level as well as word-level via projecting concepts and words into a lower dimensional space while retaining most critical semantics. In a broad context of opinion understanding system, we investigate the use of the fused embedding for several core NLP tasks: named entity detection and classification, automatic speech recognition reranking, and targeted sentiment analysis.

==> Abstract/Abstract.tex <==
\chapter* {Abstract} % '*' is to avoid the number of Chapter
% Thesis Abstract -----------------------------------------------------


Concepts are critical semantics capturing the high-level knowledge of human language. As a way to go beyond the word-level analysis, representing and leveraging the concept-level information is an important add-on to existing natural language processing (NLP) systems. More specifically, the concepts are especially critical for understanding opinions of people. For example, people express their opinion towards particular entities such products or sentiment aspects in online reviews, where these entities are actually mentions of concepts rather than merely words.  %Concepts have been given a broad definition in previous studies. In this thesis, we refined the scope of concepts to the commonsense concepts  used in our daily life and named entities belonging to a predefined set of categories. 

As compared with words, the mentions of abstract concepts may be compounded phrases (either consecutive or non-consecutive) that are likely to form a large vocabulary. Furthermore, there might be semantic properties (e.g., relations or attributes) attached to the concepts, which increases the dimensionality of concepts. In short, using concepts is faced with the curse of dimensionality. On the other hand, information from only a single level  does not suffice for a thorough understanding of human language, and meaningful representation is required at any point to encode the correlation and dependency between abstract concepts and words. In this thesis, we thus focus on effectively leveraging and integrating information from concept-level as well as word-level via projecting concepts and words into a lower dimensional space while retaining most critical semantics. In a broad context of opinion understanding system, we investigate the use of the fused embeddings for several core NLP tasks: named entity detection and classification, automatic speech recognition reranking, and targeted sentiment analysis.  

We first propose a novel method to inject the entity-based information into a word embedding space. The word embeddings are learned from a set of named entity features instead of merely contextual words. We demonstrate that the new word embeddings is a better feature representation for detecting and classifying named entities from the stream of telephone conversations. 

Apart from learning input feature embeddings, we then explore encoding the entity types  (i.e., concept categories) in a label embedding space.  Our label embeddings mainly leverage two types of information: label hierarchy and label prototype. Since our label embedding is computed prior to the training process, it has exactly the same computation complexity during runtime.   We evaluate the resulting label embeddings on multiple large scale data sets built for the task of fine-grained named entity typing. As compared with state-of-the-art methods, our label embedding method can achieve superior performance.

Next, we demonstrate that a binary embedding of the named entities can help reranking the speech-to-text hypothesis. The named entities is encoded using a Restricted Boltzman Machine (RBM) and used as a prior knowledge in the discriminative reranking model. We also extend the training of RBM to work with speech recognition hypothesis. %Evaluation on a benchmark data set shows that injecting the binary embeddings of named entity could achieve improved Word Error Rate as compared with the state-of-the-art reranking model.

Finally, we investigate on the problem of using embeddings of commonsense concepts for the task of targeted sentiment analysis. The task is also entity-centered. Namely, given a targeted entity in a sentence, the task is to resolve the correct aspects categories and corresponding sentiment polarity of the target. We propose  a new computation structure of Long Short Term Memory (LSTM) that can more effectively incorporates the embeddings of commonsense knowledge. 

In summary, this thesis proposes novel solutions of representing and leveraging concept-level and word-level information in a series of NLP tasks that are key to understanding the opinion of people.

